Towards a Paradigmatic Shift in Pre-election Polling Adequately Including Still Undecided Voters -- Some Ideas Based on Set-Valued Data for the 2021 German Federal Election

Within this paper we develop and apply new methodology adequately including undecided voters for the 2021 German federal election. Due to a cooperation with the polling institute Civey, we are in the fortunate position to obtain data in which undecided voters can state all the options they are still pondering between. In contrast to conventional polls, forcing the undecided to either state a single party or to drop out, this design allows the undecided to provide their current position in an accurate and precise way. The resulting set-valued information can be used to examine structural properties of groups undecided between specific parties as well as to improve election forecasting. For forecasting, this partial information provides valuable additional knowledge, and the uncertainty induced by the participants' ambiguity can be conveyed within interval-valued results. Turning to coalitions of parties, which is in the core of the current public discussion in Germany, some of this uncertainty can be dissolved as the undecided provide precise information on corresponding coalitions. We show structural differences between the decided and undecided with discrete choice models as well as elaborate the discrepancy between the conventional approach and our new ones including the undecided. Our cautious analysis further demonstrates that in most cases the undecideds' eventual decisions are pivotal which coalitions could hold a majority of seats. Overall, accounting for the populations' ambiguity leads to more credible results and paints a more holistic picture of the political landscape, pathing the way for a possible paradigmatic shift concerning the adequate inclusion of undecided voters in pre-election polls.

==> trash.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Different Approaches/ and theory?}

\begin{itemize}
	\item There are different approaches utilizing the valuable information of the undecided in the form of set-valued (hence partial) information.
	\begin{itemize}
		\item We compare it to the current approach neglecting all not decided individuals
		\item First: We estimate point-valued transition probabilities which can be deployed for overall estimation. (With our convenient factorization). This can be done by exploiting the information of the covariates, with some form of homogeneity assumption between the decided and the undecided
		\item Second: We reflect the uncertainty within the results with the Dempster Bounds
		\item This is also very convenient and especially relevant for coalitions (for which we hold very interesting results)
	\end{itemize}
\end{itemize}








Expected election outcome values concerning the three biggest German parties have risen and plunged within the conventional forecasts the past weeks repeatedly, questioning their accuracy concerning election outcome forecasting.


We argue that in these times the uncertainty must be communicated!
